Generative Probabilistic Novelty Detection with Adversarial Autoencoders

Novelty detection is the problem of identifying whether a new data point is considered to be an inlier or an outlier. We assume that training data is available to describe only the inlier distribution. Recent approaches primarily leverage deep encoder-decoder network architectures to compute a reconstruction error that is used to either compute a novelty score or to train a one-class classifier. While we too leverage a novel network of that kind, we take a probabilistic approach and effectively compute how likely is that a sample was generated by the inlier distribution. We achieve this with two main contributions. First, we make the computation of the novelty probability feasible because we linearize the parameterized manifold capturing the underlying structure of the inlier distribution, and show how the probability factorizes and can be computed with respect to local coordinates of the manifold tangent space. Second, we improved the training of the autoencoder network. An extensive set of results show that the approach achieves state-of-the-art results on several benchmark datasets.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We presented a approach and a network architecture for novelty detection that is based on learning mappings $f$ and $g$ that define the parameterized manifold $\mathcal{M}$ which captures the underlying structure of the inlier distribution. Unlike prior deep learning based methods, ours detects that a given sample is an outlier by computing the probability distribution. This is possible by linearizing the non-linear distribution manifold $\mathcal{M}$, and then approximate the probability density function that factorizes with respect to the local coordinates of the manifold tangent space. Our analysis showed that the method shows substantial performance increase in identifying outliers when compared with the state of the art.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

